Generative Adversarial Network based Autoencoder: Application to fault detection problem for closed loop dynamical systems

Fault detection problem for closed loop uncertain dynamical systems, is investigated in this paper, using different deep learning based methods. Traditional classifier based method does not perform well, because of the inherent difficulty of detecting system level faults for closed loop dynamical system. Specifically, acting controller in any closed loop dynamical system, works to reduce the effect of system level faults. A novel Generative Adversarial based deep Autoencoder is designed to classify datasets under normal and faulty operating conditions. This proposed network performs significantly well when compared to any available classifier based methods, and moreover, does not require labeled fault incorporated datasets for training purpose. Finally, this aforementioned network's performance is tested on a high complexity building energy system dataset.

==> sections/3a_SVM.tex <==
\subsection{Overview of SVM}
\label{SVM}

As mentioned in the previous subsection, let $x_{i}\triangleq [x_{i}^{1},\dots,x_{i}^{d}]$ denote the d-dimensional vector in input space, and let $c_{i}\in{0,1}$ denote the associated value in feature space, where $i\in[1,m]$ denotes the $i^{th}$ time instant. Let $\phi:\mathbb{R}^{d}\rightarrow\mathbb{N}$ be a mapping from the input space of $x_{i}$ to the feature space containing $c_{i}$. The objective of the SVM learning algorithm is to find a hyperplane denoted by the pair $(h_{1},h_{2})$, such that
\begin{gather}
\delta=\mathrm{min}_{i} c_{i}\bigl\{\left\langle h_{1},\phi(x_{i})\right\rangle -h_{2}\bigr\}\label{deep3}
\end{gather}
is maximized, where $\langle,\rangle$ denotes an inner product. The quantity $\bigl\{\left\langle h_{1},\phi(x_{i})\right\rangle -h_{2}\bigr\}$ denotes the distance of the input point $x_{i}$ from the decision boundary (i.e., hyperplane), and when multiplied by the label $c_{i}$ gives a positive value for a correct classification and negative for an incorrect one. If $\delta$ is positive, that means all the data points are linearly separable. Now, in \cite{cristianini2000introduction}, it is proved that for the maximal margin hyperplane, $h_{1}=\sum_{i=1}^{m} \alpha_{i}c_{i}\phi(x_{i})$, where $\alpha_{i}\in\mathbb{R}^{d}$, that maximizes $\sum_{i=1}^{m} \alpha_{i}-\sum_{i,j=1}^{m} \alpha_{i}\alpha_{j}c_{i}c_{j}\langle \phi(x_{i}),\phi(x_{j})\rangle$, subject to $\sum_{i=1}^{m}\alpha_{i}c_{i}=0,\alpha_{i}>0$. These $\alpha_{i}$ vectors are called support vectors and these are the points that lie closest to the decision boundary, i.e., maximal margin hyperplane.\par
Using (\ref{deep3}), if $\delta$ becomes negative, then the data points are not linearly separable; in that case, we can use the kernel matrix $K_{ij}$ mentioned in (\ref{deep4}). For this paper, we will use the radial basis function (RBF) kernel for classification, and try to find a nonlinear polynomial that can successfully distinguish normal and faulty data sets.

